Cross-Modal Fine-Tuning: Align then Refine

Fine-tuning large-scale pretrained models has led to tremendous progress in well-studied modalities such as vision and NLP. However, similar gains have not been observed in many other modalities due to a lack of relevant pretrained models. In this work, we propose ORCA, a general cross-modal fine-tuning framework that extends the applicability of a single large-scale pretrained model to diverse modalities. ORCA adapts to a target task via an align-then-refine workflow: given the target input, ORCA first learns an embedding network that aligns the embedded feature distribution with the pretraining modality. The pretrained model is then fine-tuned on the embedded data to exploit the knowledge shared across modalities. Through extensive experiments, we show that ORCA obtains state-of-the-art results on 3 benchmarks containing over 60 datasets from 12 modalities, outperforming a wide range of hand-designed, AutoML, general-purpose, and task-specific methods. We highlight the importance of data alignment via a series of ablation studies and demonstrate ORCA's utility in data-limited regimes.

==> tables/drug.tex <==

\begin{table}[h!]
\caption{\small Coefficient of determination  ($R^2$) results on two drug response prediction datasets. The baseline results are taken from \cite{Zhu2021ConvertingTD}. \Algo-RoBERTa  achieves better performance than the modality-specific IGTD algorithm, which converts raw tabular features into images in order to apply vision models.}
\label{table:drug}
	\centering
\begin{tabular}{lccc}
		\toprule
   Dataset   & Model  &Data representation&   $R^2$\\  
		\midrule
CTRP&	LightGBM&Tabular&		\res{0.825}{0.003}\\
&	Random forest	&Tabular 	&\res{0.786}{0.003}\\
&	CNN&	IGTD images&	\res{0.856}{0.003}\\
&	CNN&	REFINED images&	\res{0.855}{0.003}\\
&	CNN&	DeepInsight images&	\res{0.846}{0.004}\\
&	\Algo	&Tabular &	\textbf{\res{0.86}{0.002}}\\
\midrule
GDSC&	LightGBM	&Tabular &	\res{0.718}{0.006}\\
	&Random forest	&Tabular 	&\res{0.682}{0.006}\\
&	CNN&	IGTD images	&\res{0.74}{0.006}\\
&	CNN&	REFINED images	&\res{0.739}{0.007}\\
&CNN	&	DeepInsight images	&\res{0.731}{0.008}\\
&	\Algo 	&Tabular &	\textbf{\res{0.831}{0.002}}\\
		\bottomrule
	\end{tabular}

\end{table}
